Incremental Learning for Robot Perception through HRI

Scene understanding and object recognition is a difficult to achieve yet crucial skill for robots. Recently, Convolutional Neural Networks (CNN), have shown success in this task. However, there is still a gap between their performance on image datasets and real-world robotics scenarios. We present a novel paradigm for incrementally improving a robot's visual perception through active human interaction. In this paradigm, the user introduces novel objects to the robot by means of pointing and voice commands. Given this information, the robot visually explores the object and adds images from it to re-train the perception module. Our base perception module is based on recent development in object detection and recognition using deep learning. Our method leverages state of the art CNNs from off-line batch learning, human guidance, robot exploration and incremental on-line learning.

==> background.tex <==
\subsection{Incremental Learning from Humans}
In the literature, robot learning from humans is commonly named as Programming by Demonstration (PbD), Learning from Demonstration (LfD) or Imitation Learning. It should be contrasted with the automatic learning methods that do no involve active human interaction during the learning process such as reinforcement learning. The main body of work in this field focuses on learning motion trajectory from user demonstrations to perform tasks. While improving the robot's perceptual prowess is neglected in the field, still some of the fundamental challenges are shared. In particular, interfaces for information exchange and methods for incremental learning. A brief summary of research on these challenges is provided below.\\
Since the main focus in the field was to learn trajectories that were required to do actions, most interfaces are optimized to capture teacher's trajectories. Tracking human body motion \cite{kulic2008incremental} \cite{ude2004programming} \cite{kim2009stable} \cite{nakaoka2007learning}, using kinesthetic teaching where the human guides the robot to perform the task \cite{sauser2012iterative} and teleoperation where the teacher controls robots effectors directly through an interface \cite{coates2008learning} \cite{grollman2010incremental} are the main approaches for this purpose. Even though these interfaces are good for recovering the demonstrated trajectory, they are not natural in terms of human interaction. So other, more natural, interfaces were developed. Using speech \cite{cakmak2010designing}\cite{dominey2005robot} and gestures \cite{hafner2005learning} as additional information are among these. 
In most incremental learning methods, the robot uses new demonstration to bootstrap its current skill and gradually improving it \cite{zoliner2005towards}. 


\subsection{Deep Learning for Robotics}
Success of deep learning in computer vision has inspired some application in robotics. One of the main challenges of using robots in an unrestricted environment was the lack of robust and generic algorithms. Deep learning (DL) methods showed that now it is possible to achieve accurate and robust performance in many applications. Particularly, image classification and natural language processing are benefited greatly from this new technology. \\
DL models can be used as a pre-processing module, mostly on images and language, that converts raw sensor data into a lower dimensional feature space that the can be used for control. Detecting robotic grasp \cite{lenz2015deep} is using raw images to detect grasping point for various objects which can later be used for grasping. DL can also be used in an end-to-end fashion where the model is responsible for processing raw input all the way to generating control signal for the robot's effectors. Levine et al. \cite{levine2016end} implemented such network and demonstrated its feasibility by completing a few tasks. The idea of end-to-end networks for control is appealing, as it theoretically alleviates the need of detailed engineering for each module. However, it became apparent that in these networks many other hand tuning of hyper parameters and special care for training is needed and at the end they are very limited in practice. Therefore, we think that using DL enablers as modules is more practical at the moment. \\
\subsubsection{Object Localization and Detection Networks}
The goal of object localization and detection methods is to localize all the objects in a scene, commonly by bounding boxes and label them according to their class. Such methods are quite useful for scene understanding and many applications of them can be envisioned in robotics. Overfeat \cite{sermanet2013overfeat} was one of the earliest attempt for the used CNN for this task. This work used a regression network to predict a possible bounding box for an object given a grid of proposed regions with different scales. In this approach, increasing number of region proposals proved to be both crucial for accuracy and at the same time, computationally expensive. Therefore, more recent attempts\cite{ren2015faster}\cite{johnson2015densecap} utilized Region Proposal Networks (RPN) to regress bounding boxes. RPN can operate on feature maps instead of input image and by doing so, it bypasses the need for recomputing the feature maps. The details of this method will be further discussed later. 

\subsection{Multi-Class Open Set Recognition}
CNN models have achieved the state of the art in object recognition on wide variety of datasets. However, their implicit assumption is that all the possible object categories are included in the dataset. However, the situation in the real world recognition is widely different. In prediction time, the algorithm will face objects that was not in the training datasets. This is especially important for household and assistive robots. Objects in each household and work place are different and having an inclusive dataset of all of these objectes is not possible. The problem is not only about objects. For example, an assistant robot in a hospital should treat each patient differently and it needs to recognize the patient to do so. But, the current recognition methods cannot do better than recognizing the patient only as a person. \\
This problem is addressed by Incremental Machine Learning(IML) and Open Set Recognition(OSR) in literature. Main focus of the IML \cite{poggio2001incremental}\cite{crammer2006online} is to handle new instances of known classes. OSR methods \cite{scheirer2014probability}\cite{scheirer2013toward}\cite{bendale2015towards} however, need to deal with two more challenges. One is to continuously detect novel categories and two is to update the method so that it will include the new category. 












